Drag reduction in surfactant-contaminated superhydrophobic channels at high P\'eclet numbers

Motivated by microfluidic applications, we investigate drag reduction in laminar pressure-driven flows in channels with streamwise-periodic superhydrophobic surfaces (SHSs) contaminated with soluble surfactant. We develop a model in the long-wave and weak-diffusion limit, where the streamwise SHS period is large compared to the channel height and the P\'{e}clet number is large. Using asymptotic and numerical techniques, we determine the influence of surfactant on drag reduction in terms of the relative strength of advection, diffusion, Marangoni effects and bulk-surface exchange. In scenarios with strong exchange, the drag reduction exhibits a complex dependence on the thickness of the bulk-concentration boundary layer and surfactant strength. Strong Marangoni effects immobilise the interface through a linear surfactant distribution, whereas weak Marangoni effects yield a quasi-stagnant cap. The quasi-stagnant cap has an intricate structure with an upstream slip region, followed by intermediate inner regions, and a quasi-stagnant region that is mediated by weak bulk diffusion. The quasi-stagnant region differs from the immobile region of a classical stagnant cap, observed for instance in surfactant-laden air bubbles in water, by displaying weak slip. As exchange weakens, the bulk and interface decouple: the surfactant distribution is linear when the surfactant is strong, whilst it forms a classical stagnant cap when the surfactant is weak. The asymptotic solutions offer closed-form predictions of drag reduction across much of the parameter space, providing practical utility and enhancing understanding of surfactant dynamics in flows over SHSs.

==> bin.tex <==
% At high P\'{e}clet numbers, \citet{landel2020theory} established a relationship between the slip length and surfactant parameters, grating length and boundary-layer thickness. 
% The boundary-layer thickness is inversely proportional to the square (cube) root of the P\'{e}clet number in high-slip (low-slip) regimes.
% Employing long-wave and boundary-layer theories, we investigate the bulk-concentration boundary-layer and slip-length scalings outlined by \citet{landel2020theory} and \citet{temprano2023single}. 
% We predict drag reduction in both high-slip and low-slip regimes, without the need for empirical coefficient fitting and expensive numerical simulations. 
% Our analysis reveals the intricate structure of the boundary layer that can arise when both Marangoni and diffusive effects are weak.
% The amount of surfactant at the interface must be prescribed for insoluble surfactants, whereas, for soluble surfactants, it is mediated by bulk diffusion, which allows the cap to come into equilibrium with the bulk concentration.
% In \S\ref{sec:asymptotic}, we derive asymptotic results.
% We find analytical solutions for the surfactant distribution and drag reduction in both high-slip and low-slip regimes.
% Surfactants adsorb onto the interface, are advected by the channel flow, and accumulate at the downstream stagnation point, changing the interfacial stress and generating a Marangoni effect that increases the drag.
% For $\epsilon \ll 1$, this non-dimensionalisation results in a long-wave theory in the streamwise direction with a dominant streamwise flow.
% Next, we substitute the non-dimensionalisation \eqref{eq:nondimensionalisation} into the governing equations and boundary conditions \eqref{eq:dimensional_equations}--\eqref{eq:dimensional_drag}. 
% \begin{equation}
% 	\hat{u}_{\hat{x}} + \hat{v}_{\hat{y}} = 0, \quad \hat{\mu} \hat{\nabla}^2 \hat{u}-  \hat{p}_{\hat{x}} = 0, \quad \hat{\mu} \hat{\nabla}^2 \hat{v}- \hat{p}_{\hat{y}} = 0, \quad
% 	\hat{D} \hat{\nabla}^2 \hat{c} - \hat{u} \hat{c}_{\hat{x}} - \hat{v} \hat{c}_{\hat{y}} = 0, \tag{\theequation\textit{a--c}}
% \end{equation}
% \begin{multline}
% 	\frac{\hat{U}}{\hat{P}} u_x + \frac{\hat{U}}{\hat{P}} v_{y} = 0, \\ \frac{\hat{\mu}\hat{U}}{\hat{P}^2} u_{xx} + \frac{\hat{\mu}\hat{U}}{\epsilon^2 \hat{P}^2} u_{yy} - \frac{\hat{\mu}\hat{U}}{\epsilon \hat{H}\hat{P}} p_x = 0, \quad \frac{\epsilon\hat{\mu}\hat{U}}{\hat{P}^2} v_{xx} + \frac{\epsilon\hat{\mu}\hat{U}}{\epsilon^2 \hat{P}^2} v_{yy} - \frac{\hat{\mu}\hat{U}}{\epsilon^2 \hat{H} \hat{P}} p_y = 0, \\
% 	\frac{\hat{D}\hat{C}}{\hat{P}^2} c_{xx} + \frac{\hat{D}\hat{C}}{\epsilon^2 \hat{P}^2} c_{yy} - \frac{\hat{U} \hat{C}}{\hat{P}} u c_x - \frac{\epsilon \hat{U} \hat{C}}{\epsilon \hat{P}} v c_y = 0, \tag{\theequation\textit{a--c}}
% \end{multline}
% \begin{multline}
% 	u_x + v_{y} = 0, \\ \frac{\hat{\mu}\hat{U}}{\hat{P}^2} u_{xx} + \frac{\hat{\mu}\hat{U}}{\epsilon^2 \hat{P}^2} u_{yy} - \frac{\hat{\mu}\hat{U}}{\epsilon^2 \hat{P}^2} p_x = 0, \quad \frac{\epsilon\hat{\mu}\hat{U}}{\hat{P}^2} v_{xx} + \frac{\epsilon\hat{\mu}\hat{U}}{\epsilon^2 \hat{P}^2} v_{yy} - \frac{\hat{\mu}\hat{U}}{\epsilon^3 \hat{P}^2} p_y = 0, \\
% 	\frac{\hat{D}\hat{C}}{\hat{P}^2} c_{xx} + \frac{\hat{D}\hat{C}}{\epsilon^2 \hat{P}^2} c_{yy} - \frac{\hat{U} \hat{C}}{\hat{P}} u c_x - \frac{\hat{U} \hat{C}}{\hat{P}} v c_y = 0, \tag{\theequation\textit{a--c}}
% \end{multline}
% \begin{multline}
% 	u_x + v_{y} = 0, \quad \epsilon^2 u_{xx} + u_{yy} - p_x = 0, \\ \epsilon^4 v_{xx} + \epsilon^2 v_{yy} - p_y = 0, \quad
% 	\epsilon^2 \frac{\hat{D}}{\hat{P}\hat{U}} c_{xx} + \frac{\hat{D}}{\hat{P} \hat{U}} c_{yy} - \epsilon^2 u c_x - \epsilon^2 v c_y = 0, \tag{\theequation\textit{a--c}}
% \end{multline}
% \begin{multline}
% 	\frac{\hat{\mu}\hat{U}}{\epsilon \hat{P}} u_y - \frac{ \hat{A} \hat{G}}{\hat{P}} \Gamma_{x} = 0, \quad \epsilon \hat{U} v =0, \quad \frac{\hat{D}\hat{C}}{\epsilon \hat{P}} c_y - \hat{K}_a \hat{C} c + \frac{\hat{K}_d \hat{K}_a \hat{C}}{\hat{K}_d}\Gamma  =0, \\ \quad  \frac{\hat{D}_I \hat{K}_a \hat{C}}{\hat{P}^2 \hat{K}_d} \Gamma_{xx} + \hat{K}_a \hat{C} c -  \frac{\hat{K}_d\hat{K}_a\hat{C}}{\hat{K}_d} \Gamma  - \frac{\hat{U} \hat{K}_a \hat{C}}{\hat{P}\hat{K}_d}(u \Gamma)_{x} = 0,
%     \tag{\theequation\textit{a--e}}
% \end{multline}
% \begin{multline}
% 	u_y - \epsilon \frac{ \hat{A} \hat{G}}{\hat{\mu}\hat{U}} \Gamma_{x} = 0, \quad v =0, \quad  c_y - \frac{\hat{K}_a\hat{H}}{\hat{D}} (c - \Gamma)  =0, \\ \quad  \frac{\hat{D}_I}{\hat{P} \hat{U}} \Gamma_{xx} + \frac{\hat{P}\hat{K}_d}{\hat{U}}( c - \Gamma)  - (u \Gamma)_{x} = 0,
%     \tag{\theequation\textit{a--e}}
% \end{multline}
% \begin{equation}
%     \hat{U} \hat{G} u \Gamma - \frac{\hat{D}_I\hat{G}}{\hat{P}} \Gamma_{x} = 0,
% \end{equation}
% \begin{equation}
%     u \Gamma - \frac{\hat{D}_I}{\hat{P}\hat{U}} \Gamma_{x} = 0,
% \end{equation}
% \begin{equation}
%     u \Gamma - \frac{\epsilon\hat{D}_I}{\hat{H}\hat{U}} \Gamma_{x} = 0,
% \end{equation}
% \refstepcounter{equation} 
% \begin{multline}
%     \frac{\text{d}}{\text{d}x} \int_{y=0}^{2} (\frac{\epsilon \hat{U}\hat{C}}{1} u c - \frac{\epsilon \hat{D} \hat{C}}{\hat{P}} c_x) \, \text{d} y  = (\frac{\hat{K}_d \hat{K}_a \hat{C}}{\hat{K}_d} \Gamma - \frac{\hat{K}_a\hat{C}}{1} c), \\ 
%     \frac{\text{d}}{\text{d}x}(\frac{\hat{U}\hat{K}_a\hat{C}}{\hat{P}\hat{K}_d}u \Gamma - \frac{\hat{D}_I\hat{K}_a\hat{C}}{\hat{P}^2\hat{K}_d} \Gamma_{x}) = - (\frac{\hat{K}_d \hat{K}_a \hat{C}}{\hat{K}_d} \Gamma - \frac{\hat{K}_a\hat{C}}{1} c), \\ 
%     \hat{K} = \int_{y=0}^{2} \frac{\epsilon \hat{P} \hat{U}\hat{C}}{1} u c - \frac{\epsilon \hat{D} \hat{C}}{1} c_x \, \text{d}y + (\frac{\hat{U}\hat{K}_a\hat{C}}{\hat{K}_d} u \Gamma - \frac{\hat{D}_I\hat{K}_a\hat{C}}{\hat{P}\hat{K}_d}  \Gamma_{x}), \\
%     \int_{x=-\phi }^{\phi} (\frac{\hat{K}_d \hat{K}_a \hat{C}\hat{P}}{\hat{K}_d}  \Gamma - \frac{\hat{K}_a\hat{C}\hat{P}}{1} c) \, \text{d}x = 0, \tag{\theequation\textit{a--d}}
% \end{multline}
% \refstepcounter{equation} 
% \begin{multline} 
%     \frac{\text{d}}{\text{d}x} \int_{y=0}^{2} (\frac{\epsilon \hat{U}}{1} u c - \frac{\epsilon \hat{D}}{\hat{P}} c_x) \, \text{d} y  = (\frac{\hat{K}_a}{1} \Gamma - \frac{\hat{K}_a}{1} c), \\ 
%     \frac{\text{d}}{\text{d}x}(\frac{\hat{U}}{\hat{P}\hat{K}_d}u \Gamma - \frac{\hat{D}_I}{\hat{P}^2\hat{K}_d} \Gamma_{x}) = - (\frac{1 }{1} \Gamma - \frac{1}{1} c), \\ 
%     1 = \int_{y=0}^{2} \frac{\epsilon \hat{P} \hat{U}}{\hat{Q}} u c - \frac{\epsilon \hat{D}}{\hat{Q}} c_x \, \text{d}y + (\frac{\hat{U}\hat{K}_a}{\hat{K}_d \hat{Q}} u \Gamma - \frac{\hat{D}_I\hat{K}_a}{\hat{P}\hat{K}_d \hat{Q}}  \Gamma_{x}), \\
%     \int_{x=-\phi }^{\phi} (\Gamma - c) \, \text{d}x = 0, \tag{\theequation\textit{a--d}}
% \end{multline}
% \refstepcounter{equation}
% \begin{multline} 
%     \frac{\text{d}}{\text{d}x} \int_{y=0}^{2} ( u c - \frac{\hat{D}}{\hat{P}\hat{U}} c_x) \, \text{d} y  = (\frac{\hat{K}_a}{\epsilon \hat{U}} \Gamma - \frac{\hat{K}_a}{\epsilon \hat{U}} c), \\ 
%     \frac{\text{d}}{\text{d}x}(u \Gamma - \frac{\hat{D}_I}{\hat{P} \hat{U}} \Gamma_{x}) = - (\frac{\hat{P} \hat{K}_d }{\hat{U}} \Gamma - \frac{\hat{P} \hat{K}_d}{\hat{U}} c), \\ 
%     1 = \int_{y=0}^{2} u c - \frac{\epsilon \hat{D}}{\hat{H}\hat{U}} c_x \, \text{d}y + \frac{\hat{K}_a}{\hat{K}_d \hat{H}} ( u \Gamma - \frac{\hat{D}_I}{\hat{P}\hat{U}}  \Gamma_{x}), \\
%     \int_{x=-\phi }^{\phi} (\Gamma - c) \, \text{d}x = 0, \tag{\theequation\textit{a--d}}
% \end{multline}
% \begin{multline}
% 	u_x + v_{y} = 0, \quad \epsilon^2 u_{xx} + u_{yy} - p_x = 0, \\ \epsilon^4 v_{xx} + \epsilon^2 v_{yy} - p_y = 0, \quad
%     \frac{1}{\mathscr{P}}\left(\epsilon^2 c_{xx} + c_{yy}\right) - u c_x -v c_y = 0,
%     \tag{\theequation\textit{a--c}}
% \end{multline}
% \begin{multline}
% 	u_y - \mathscr{M} \Gamma_{x} = 0, \quad v =0, \quad c_y - \Da (c -\Gamma)  =0, \\ \quad \frac{\epsilon^2 \Gamma_{xx}}{\mathscr{P}_I} + \mathscr{B} ( c - \Gamma)  - (u \Gamma)_{x} = 0,
%     \tag{\theequation\textit{a--e}}
% \end{multline}
% At $x = \pm \phi$ and $y=0$, the no-flux condition \eqref{eq:nondimensional_noflux} is dominated by advection 
% \begin{equation}
%     u \Gamma - \frac{\epsilon^2 \Gamma_{x}}{\mathscr{P}_I} = 0.
% \end{equation}
% \begin{equation}\label{eq:nondimensional_noflux_0_wd}
%     u_0 \Gamma_0 = 0.
% \end{equation}
% We do not resolve these here, as it is sufficient to impose continuity conditions $\boldsymbol{u}_0(\phi^-,\,y) = \boldsymbol{u}_0(\phi^+,\,y)$ and $\boldsymbol{u}_0(-\phi,\,y) = \boldsymbol{u}_0(2- \phi,\,y)$ are imposed between $\mathcal{D}_1$ and $\mathcal{D}_2$. 
% \begin{subequations} 
% \begin{align}
%     \frac{\text{d}}{\text{d}x} \int_{y=0}^{2} \left( u c - \frac{\epsilon^2 c_x}{\mathscr{P}} \right) \, \text{d} y  - \frac{\Da}{\mathscr{P}}(\Gamma - c) &= 0, \\ 
%     \frac{\text{d}}{\text{d}x}\left(u \Gamma - \frac{\epsilon^2 \Gamma_{x}}{\mathscr{P}_I} \right) + \mathscr{B}( \Gamma - c) &= 0, \\ 
%     \int_{y=0}^{2} \left( u c - \frac{\epsilon^2 c_x}{\mathscr{P}}\right) \, \text{d}y + \frac{\Da}{\mathscr{B}\mathscr{P}} \left( u \Gamma - \frac{\epsilon^2 \Gamma_{x}}{\mathscr{P}_I}\right) &= 1, 
% \end{align}
% \end{subequations}
% In $\mathcal{D}_2$, surfactant transport is dominated by advection, so that \eqref{eq:nd_fluxes_d2} becomes
% % \refstepcounter{equation}
% % \begin{equation}
% %     \frac{\text{d}}{\text{d}x} \int_{ y=0}^{2} \left(u c - \frac{\epsilon^2 c_x}{\mathscr{P}} \right) \, \text{d}y  = 0, \quad \int_{y=0}^{2} \left(u c - \frac{\epsilon^2 c_x}{\mathscr{P}} \right) \, \text{d}y = 1, 
% % \end{equation}
% \begin{equation} \label{eq:nd_fluxes_d2_0_wd}
%     \int_{y=0}^{2} u_0 c_0 \, \text{d}y = 1. 
% \end{equation}
% Solvability conditions can be derived from the first-order system which constrains the variables at leading order \citep{tomlinson2023laminar} .
% However, these conditions are equivalent to the leading-order volume and surfactant-flux conditions provided in (\ref{eq:nd_fluxes_d1_0_wd}, \ref{eq:nd_velocity_flux_0_wd}).
% \refstepcounter{equation} \label{eq:c_bvp_1_wd} 
% \begin{multline}
% 	\alpha (\epsilon^2 c_{0xx} + c_{0yy}) - (\tilde{U} p_{0x} + (\gamma / \beta) \bar{U}\Gamma_{0x}) c_{0x} - (\tilde{V} p_{0xx} + ( \gamma / \beta) \bar{V}\Gamma_{0xx}) c_{0y} = 0 \quad \text{in} \quad \mathcal{D}_1,  \\
%     \alpha (\epsilon^2 c_{0xx} + c_{0yy}) - \breve{U} p_{0x} c_{0x} - \breve{V} p_{0xx} c_{0y} = 0 \quad \text{in} \quad \mathcal{D}_2, \tag{\theequation\textit{a,\,b}}
% \end{multline}
% OR
% \begin{multline}
% 	\alpha (\epsilon^2 c_{0xx} + c_{0yy}) - (\tilde{U} (1/\tilde{Q} - (\gamma/\beta)(\bar{Q}/\tilde{Q})\Gamma_{0x})) + (\gamma / \beta) \bar{U}\Gamma_{0x}) c_{0x} \\ 
%  - (\tilde{V} (-(\gamma/\beta)(\bar{Q}/\tilde{Q})\Gamma_{0xx}) + ( \gamma / \beta) \bar{V}\Gamma_{0xx}) c_{0y} = 0 \quad \text{in} \quad \mathcal{D}_1,  \\
%     \alpha (\epsilon^2 c_{0xx} + c_{0yy}) - \breve{U} (1/\breve{Q}) c_{0x} = 0 \quad \text{in} \quad \mathcal{D}_2, \tag{\theequation\textit{a,\,b}}
% \end{multline}
% \refstepcounter{equation} \label{eq:c_bvp_2_wd} 
% \begin{equation} 
%     c_{0y} - (\nu/ \alpha)(c_0 - \Gamma_0) = 0, \quad \nu ( c_0 - \Gamma_0)  - ((\beta \tilde{U} p_{0x} +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 - \epsilon^2 \delta \Gamma_{0x})_{x} = 0, \tag{\theequation\textit{a,\,b}}
% \end{equation}
% OR 
% \begin{equation}  
%     (\beta \tilde{U} p_{0x} +\gamma \bar{U}\Gamma_{0x}) \Gamma_0 - \epsilon^2 \delta \Gamma_{0x} = 0.
% \end{equation}
% The system in \eqref{eq:c_bvp_1_wd}--\eqref{eq:c_bvp_6_wda} can be entirely expressed in terms of the unknowns $c_0$ and $\Gamma_0$, using the volume-flux conditions \eqref{eq:c_bvp_8_wd}. 
% The reduction of the problem from a seven-parameter Stokes-flow system \eqref{eq:nondimensional_equations}--\eqref{eq:nd_velocity_flux} for five variables, to the seven-parameter long-wave system \eqref{eq:c_bvp_1_wd}--\eqref{eq:c_bvp_6_wda} for two variables, to the five-parameter system for two variables (when we neglect streamwise diffusion in the bulk and at the interface in \eqref{eq:c_bvp_1_wd}--\eqref{eq:c_bvp_6_wda}), simplifies the problem's solution. 
% such that $\bar{c}_0 = \bar{c}_0(x)$.
% \begin{subequations} \label{eq:c_bvp_6_sd} 
% \begin{align}
%     \frac{\text{d}}{\text{d}x} (\tilde{Q} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) + (\gamma / \beta) \bar{Q}\Gamma_{0x}) c_0 - \nu(\Gamma_0 - c_0) &= 0, \\
%     \frac{\text{d}}{\text{d}x} (\beta \tilde{U} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 + \nu ( \Gamma_0 - c_0) &= 0, \\ 
%     (\tilde{Q} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) + (\gamma / \beta) \bar{Q}\Gamma_{0x}) c_0 + (\beta \tilde{U} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 &= 1,
% \end{align}
% \end{subequations}
% \begin{subequations} \label{eq:c_bvp_6_sd} 
% \begin{align}
%     c_{0x} - \nu(\Gamma_0 - c_0) &= 0, \\
%     \frac{\text{d}}{\text{d}x} (\beta \tilde{U} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 + \nu ( \Gamma_0 - c_0) &= 0, \\ 
%     c_0 + (\beta \tilde{U} (1/\tilde{Q} - (\gamma / \beta)\bar{Q}\Gamma_{0x}/\tilde{Q}) +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 &= 1,
% \end{align}
% \end{subequations}
% \begin{subequations} \label{eq:c_bvp_6_sd} 
% \begin{align}
%     c_{0x} - \nu(\Gamma_0 - c_0) &= 0, \\
%     \frac{\text{d}}{\text{d}x} (\beta \tilde{U} / \tilde{Q} - \gamma \tilde{U} \bar{Q}\Gamma_{0x}/\tilde{Q} +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 + \nu ( \Gamma_0 - c_0) &= 0, \\ 
%     c_0 + (\beta \tilde{U} /\tilde{Q} - \gamma \tilde{U} \bar{Q}\Gamma_{0x}/\tilde{Q}) +  \gamma \bar{U}\Gamma_{0x}) \Gamma_0 &= 1,
% \end{align}
% \end{subequations}
% \begin{subequations} \label{eq:c_bvp_6_sd} 
% \begin{align}
%     c_{0x} - \nu(\Gamma_0 - c_0) &= 0, \\
%     \frac{\text{d}}{\text{d}x} ((3/4) \beta - (1/2) \gamma \Gamma_{0x}) \Gamma_0 + \nu ( \Gamma_0 - c_0) &= 0, \\ 
%     c_0 + ((3/4) \beta - (1/2) \gamma \Gamma_{0x}) \Gamma_0 &= 1,
% \end{align}
% \end{subequations}
% Equation (\ref{eq:c_bvp_6_sd}\textit{c}) is the flux constraint imposed on the $x$-integral of the sum of (\ref{eq:c_bvp_6_sd}\textit{a}) and (\ref{eq:c_bvp_6_sd}\textit{b}).
% \sout{Note that the ``1D long-wave model'' in \eqref{eq:c_bvp_6_sd} is derived for a 2D channel flow, whereas, the ``1D long-wave model'' was derived for a 3D channel flow\mbox{\citep{tomlinson2023laminar}}, resulting in different transport coefficients.}
% \textit{The drag-reduction map (figure \ref{fig:12}\textit{c}) is partitioned into three regions based on the strength of cross-channel diffusion.
% Asymptotic solutions are derived when cross-channel diffusion is weak (strong) for $\alpha\ll1$ ($\alpha \gg 1)$ using the 2D (1D) model in \S\ref{sec:asymptotic} \cite[Appendix C in][]{tomlinson2023laminar}, yielding the black dashed lines for $\alpha \in [0.01, \, 0.1]$ ($\alpha \in [10, \, 100]$) in figure \ref{fig:12}.
% The $c_0$ and $\Gamma_0$ associated with these changes in ${DR}_0$ are depicted in figure \ref{fig:12}(\textit{a--b}) for $\gamma = 1$ and figure \ref{fig:12}(\textit{f--g}) for $\gamma = 0.1$.
% }
% In figure S1 of the supplementary material, we present plots of $c_0$ and $\Gamma_0$ at several different locations across parameter space: $\alpha = 0.1$, $1$, $10$ and $100$.
% We bound region $A^\textsl{2D}$ using a similar condition below. 
% using black dashed lines.

% \textit{From figure \ref{fig:12}(\textit{a}) to \ref{fig:12}(\textit{b}), the gradient and magnitude of $\Gamma_0$ decreases as advection and then diffusion dominates over Marangoni effects.
% Advection leads to surfactant accumulation at the downstream end of the interface, reducing the surfactant gradient over the rest of the interface, while diffusion spreads the accumulated surfactant over the downstream end of the interface. 
% % Both transport processes contribute to reducing the drag.
% As $\alpha$ decreases, there is less variation in $\langle c_0 \rangle$ along the period but more variation in $c_0$ across the channel, as the surfactant dynamics take place inside a bulk-concentration boundary layer close to the SHS.}
% \st{\begin{multline}
%     \Gamma_0(-\phi)=0 \Rightarrow \frac{3\beta}{2\gamma}(-\phi - x_0)=0 \Rightarrow x_0 = -\phi \Rightarrow 2 \phi = 2 \phi a_1 \gamma^{3/5} / \alpha^{1/10} \\ 2 \phi = (2 \phi \gamma^{3/5} / \alpha^{1/10})((-5\lambda/(6C'(0))^{3/5}/(2\phi)) \Rightarrow 2\phi = 0 \quad \text{as} \quad \lambda =0.
% \end{multline}
% so what is going on here?} 
%In this limit, the slip, deceleration and transition regions discussed in \st{Appendix \ref{sec:asymptotic_a}} collapse around $x = -\phi$. 
%Hence, we use an asymptotic condition to give a boundary for region $A^\textsl{2D}$, such that $\Gamma_0(-\phi)=0$ when $\gamma \sim \alpha^{1/6}$ and $a_1 \sim 1$.
%As $\gamma \approx 0.7$ and $1$ for $\alpha = 0.1$ and $1$ in figure \ref{fig:12}(\textit{g}), the boundary between regions $M^\textsl{2D}$ and $A^\textsl{2D}$ is similar whether we approach from large or small $\gamma$. 
% Increasing diffusion recovers a 1D bulk concentration profile and eliminates the quasi-stagnant cap (figure \ref{fig:12}\textit{j,\,k}).

% \textit{From figure \ref{fig:12}(\textit{f}) to \ref{fig:12}(\textit{g}), the thickness and amplitude of the upstream and downstream boundary layers in $\Gamma_0$ and $c_0(x, \,0)$ are attenuated by streamwise diffusion. }
%and consequently $v_0$ shows a minor deviation from zero because of surfactant effects.
% The surfactant gradient exhibits weak variation along the liquid--gas interface. 
%We identify an advection--dominated region with weak exchange and a bulk concentration boundary layer ($A^\textsl{2D}_{E}$, figure \ref{fig:dr_shems}\textit{b}) when $\alpha \ll 1$, such that (\S\ref{subsec:MA_WE})
%, where $\epsilon^2 \alpha = \epsilon^2 \delta$, $\beta = 1$ and 
% In the subsequent subsections, we examine flow and surfactant field in the strong- and weak-cross-channel-diffusion regions, characterised by $\alpha \gg 1$ and $\alpha \ll 1$. 
% Notably, the drag-reduction behaviour in the weak-cross-channel-diffusion region has changed from $\nu = 100$ (figure \ref{fig:12}\textit{c--e}) to $\nu = 0.01$ (figure \ref{fig:11}\textit{c--e}). 

%We investigate $c_0$ and $\Gamma_0$ in different regions of the drag-reduction map in figure \ref{fig:11}(\textit{c--e}), for $\gamma = 1$ in figure \ref{fig:11}(\textit{a}--\textit{b}) and for $\gamma = 0.1$ in figure \ref{fig:11}(\textit{f}--\textit{g}).
%Asymptotic solutions, detailed in \S\ref{subsec:MA_WE} \cite[Appendix D in][]{tomlinson2023laminar}, yield the black dashed lines that are plotted for $\alpha \in [0.1, \, 10]$ ($\alpha \in [10, \, 100]$) in figure \ref{fig:12}.
% Additional plots of $c_0$, $\Gamma_0$ and $K_0$ at $\alpha = 0.1$, $1$, $10$ and $100$ are given in figure S3 of the supplementary material.

% \subsubsection{Strong cross-channel diffusion} \label{sec:scd2}


% \subsubsection{Weak cross-channel diffusion} \label{sec:wcd2}

% As the bulk--surface exchange strength decreases from figures \ref{fig:12}(\textit{c--e}) to \ref{fig:11}(\textit{c--e}), we observe a transition in drag-reduction behaviour from ${DR}_0 = O(\gamma^{6/10}/\alpha^{1/10})$ (strong exchange) to ${DR}_0 = O(\gamma^{1/2})$ (weak exchange) when cross-channel diffusion is weak, and the drag-reduction contours level out.

% In figure \ref{fig:11}(\textit{c,\,d,\,e,\,f}), dashed black asymptotes for $c_0$, $\Gamma_0$ and ${DR}_0$ when $\alpha \in[0.1,\,1]$ are plotted using (\ref{eq:a_we}\textit{a--c}). 
% Similar to the strong-exchange problem, decreasing $\alpha$ from figure \ref{fig:11}(\textit{b}) to \ref{fig:11}(\textit{a}) increases the surfactant gradient at the liquid--gas interface. 
% We transition from region $M^\textsl{2D}_{E}$ to region $A^\textsl{2D}_{E}$ when $\gamma = O(1)$. 
% Decreasing the surfactant strength means that advection dominates over Marangoni effects and the surfactant accumulates within a boundary layer at the downstream end of the liquid--gas interface. 
% By decreasing $\alpha$ from figure \ref{fig:11}(\textit{g}) to \ref{fig:11}(\textit{f}) the surfactant profile transitions into the classical stagnant-cap regime \citep{he1991size}, which we describe alongside the velocity field in the next paragraph. 
% Here, the streamwise velocity closely resembles a no-slip flow, indicating that the wall-normal flow is minimal and there is little curving of streamlines over the interface. 
% For each experiment, we overlay the data point evaluated below onto the summary of asymptotic predictions for the leading-order drag reduction in the 2D long-wave model (figure \ref{fig:11}). 
% Specifically, for 
% \citet{song2018effect}: $\alpha \approx 5\times10^{-3}$, $1\times 10^{-1} \lessapprox \gamma \lessapprox 6.8\times 10^{1}$ ($A^\textsl{2D}M^\textsl{2D}$ boundary, figure \ref{fig:dr_shems}); 
% We have explored how the interfacial concentration ($\Gamma_0$), bulk concentration ($c_0$) and leading-order drag reduction (${DR}_0$) are influenced by bulk diffusion ($\alpha$), surface advection ($\beta$), surfactant strength ($\gamma$), interfacial diffusion ($\delta$) and bulk--surface exchange ($\nu$).
% In cases where cross-channel diffusion dominates, we recover the Marangoni-dominated ($M^\textsl{1D}$) and diffusion-dominated ($D^\textsl{1D}$) regions identified in \citet{tomlinson2023laminar} (figures \ref{fig:12} and \ref{fig:11}).  
% In region $M^\textsl{1D}$, the interface is immobilised, resulting in ${DR}_0 \sim \epsilon^2\alpha/\gamma \ll 1$ for $\alpha \gg \epsilon^2$ and ${DR}_0 \sim \phi/\gamma \ll 1$ for $1\ll \alpha \ll \epsilon^2$, while in region $D^\textsl{1D}$, the interface is shear-free, yielding $1 - {DR}_0 \sim \gamma /\epsilon^2\alpha \ll 1$.
% The quantities 
% $${DR}_0\sim\frac{\epsilon^2\alpha}{\gamma} \sim \epsilon^2  \cdot\frac{\hat{D}\hat{P}}{\hat{Q}\hat{H}}\cdot\frac{\hat{\mu}\hat{K}_d^2\hat{P}\hat{Q}^2}{\hat{A}\hat{H}\hat{K}\hat{K}_a^2} \sim \frac{\epsilon \hat{D}\hat{\mu}\hat{k}_d^2 \hat{P}}{\hat{A}\hat{H}\hat{\Gamma}_m^2\hat{k}_a^2\hat{c}_0} \sim \frac{\epsilon \hat{P} \hat{H}}{\hat{L}_m^2} \quad \frac{[m^2]}{[m^2]}$$ 
% $\epsilon^2\alpha/\gamma \sim \hat{H}^2/\hat{L}_m^2$ 
% and 
% $${DR}_0\sim\frac{\phi}{\gamma} \sim \phi \cdot \frac{\hat{\mu}\hat{K}_d^2\hat{P}\hat{Q}^2}{\hat{A}\hat{H}\hat{K}\hat{K}_a}\sim \frac{\phi \hat{\mu}\hat{k}_d^2\hat{P}\hat{Q}}{\hat{n}\hat{R}\hat{T}\hat{H}\hat{\Gamma}_m^2\hat{k}_a^2\hat{c}_0} \sim \frac{\phi \hat{P} \hat{H}}{\hat{L}_m^2} \cdot \frac{\hat{Q}}{\hat{D}} \quad \frac{[m^2]}{[m^2]} \cdot\frac{[m^2/s]}{[m^2/s]}$$
% $\phi/\gamma \sim (\phi \hat{P} \hat{H}/\hat{L}_m^2) (\hat{Q}/\hat{D})$,
% where 
% $$\hat{L}_m^2 = \frac{\hat{n}\hat{R}\hat{T} \hat{H}^2\hat{\Gamma}_m^2\hat{k}_a^2 \hat{c}_0}{\hat{D}\hat{\mu}\hat{k}_d^2} \quad \frac{[m\,kg\,s^{-3}]}{[m\,kg\,s^{-3}]}$$
% $\hat{L}_m^2 = (\hat{n}\hat{R}\hat{T} \hat{H}^2\hat{\Gamma}_m^2\hat{\kappa}_a^2 \hat{c}_0)/(\hat{D}\hat{\mu}\hat{\kappa}_d^2)$
% is the mobilisation length defined in \citet{temprano2023single}, $\hat{K}_a = \hat{\Gamma}_m \hat{\kappa}_a$ and $\hat{K}_d = \hat{\kappa}_d$. 
% Using \eqref{eq:slip} for ${DR}_0 \ll 1$, the slip length $\lambda_0 \sim \epsilon \phi P / L_m^2$ for $\alpha \gg \epsilon^2$ and $\lambda_0 \sim \epsilon \phi^2 P^2 / L_m^2$ for $1\ll \alpha \ll \epsilon^2$, where $P = \hat{P}/\hat{H}$, $L_m = \hat{L}_m/\hat{H}$ and $\hat{Q}/\hat{D}=O(1)$.
% Hence, when $1 \ll \alpha \ll \epsilon^2$, we recover the grating- and mobilisation-length scalings derived in \citet{temprano2023single} with $\lambda_e \sim \lambda_0/\epsilon$, and when $\alpha \gg \epsilon^2$, we find a weaker dependence on $\phi P$ due to strong cross-channel diffusion.
% Conversely, when $1 - {DR}_0 \ll 1$, \eqref{eq:slip} gives $\lambda_0 = (\Delta p_I - \Delta p_U) / (\Delta p_I \Delta p_U)$.
% However, under weak cross-channel diffusion and strong exchange, we unveil new subregions, $M^\textsl{2D}$ and $A^\textsl{2D}$.
% In these regions, a bulk concentration boundary layer forms, influencing the drag reduction when bulk--surface exchange is strong (figure \ref{fig:12}).
% Specifically, in $M^\textsl{2D}$, ${DR}_0 \sim \phi^{5/3} \alpha^{2/3}/\gamma \ll 1$, characterised by a linear interfacial-surfactant distribution, whereas in $A^\textsl{2D}$, $1-{DR}_0 \sim \gamma^{6/10}/\alpha^{1/10} \ll 1$, featuring a quasi-stagnant cap interfacial-surfactant distribution. 
% The quantity 
% \begin{multline}\frac{\phi^{5/3} \alpha^{2/3}}{\gamma} 
% \sim \phi^{5/3} \cdot \frac{\hat{D}^{2/3}\hat{P}^{2/3}}{\hat{Q}^{2/3}\hat{H}^{2/3}}\cdot\frac{\hat{\mu}\hat{K}_d^2\hat{P}\hat{Q}^2}{\hat{A}\hat{H}\hat{K}\hat{K}_a^2} \sim \frac{\hat{D}^{2/3}\hat{\mu}\hat{k}_d^2 \hat{P}^{5/3} \hat{Q}^{1/3}}{\hat{A}\hat{H}^{5/3}\hat{\Gamma}_m^2\hat{k}_a^2\hat{c}_0} \\ \sim \frac{\phi^{5/3}\hat{P}^{5/3}\hat{H}^{1/3}}{L_m^2} \cdot \frac{\hat{Q}^{1/3}}{\hat{D}^{1/3}} \quad \frac{[m^2]}{[m^2]}\cdot \frac{[m^2/s]}{[m^2/s]},\end{multline}
% $\phi^{5/3} \alpha^{2/3}/\gamma 
% \sim (\phi^{5/3}\hat{P}^{5/3}\hat{H}^{1/3}/L_m^2)(\hat{Q}^{1/3}/\hat{D}^{1/3}),$
% such that using \eqref{eq:slip} for ${DR}_0 \ll 1$, we have that $\lambda_0 \sim \epsilon \phi^{8/3} P^{8/3} / L_m^2 $ for $\alpha \ll 1$.
% Hence, when $\alpha \ll 1$, we find that $\lambda_e$ has a stronger dependence on $\phi P$ than \citet{temprano2023single} due to weak cross-channel diffusion.
% Conversely, when bulk--surface exchange is weak, we identify subregions $M^\textsl{2D}_E$ and $A^\textsl{2D}_E$.
% ${DR}_0 \sim 1/\gamma \ll 1$ in $M^\textsl{2D}_E$, with a linear interfacial-surfactant distribution, and $1 - {DR}_0 \sim\gamma^{1/2} \ll 1$ in $A^\textsl{2D}_E$, where the interfacial-surfactant distribution forms a classical stagnant cap (figure \ref{fig:11}).    
% These asymptotic solutions for ${DR}_0$ are summarised in figure \ref{fig:dr_shems}.
% % Drag reduction can be achieved by enhancing diffusion (moving into region $M^\textsl{1D}$, $A^\textsl{1D}$ or $D^\textsl{1D}$ for strong exchange or $M^\textsl{1D}_E$ or $A^\textsl{1D}_E$ or $D^\textsl{1D}_E$ for weak exchange) or by diminishing surfactant strength (moving into region $D^\textsl{1D}$, $A^\textsl{1D}$ or $A^\textsl{2D}$ for strong exchange or $D^\textsl{1D}_E$, $A^\textsl{1D}_E$ or $A^\textsl{2D}_E$ for weak exchange).% We now outline our assumptions as future extensions of our model.
% Firstly, we have assumed that $\epsilon \ll 1$, which simplifies Stokes equations.
% Without this assumption, simulations of the full equations would have to be done in COMSOL \citep{landel2020theory}. 
% Secondly, we have linearised the equation of state and adsorption--desorption kinetics, however, there does exist studies which consider insoluble surfactant with non-linear equations of state \cite[e.g.][]
% {mayer2022superhydrophobic}.
% Thirdly, we have assumed that the ridges are filled with gas, however, there does exist studies which consider liquid-infused channels \cite[e.g.][]
% {sundin2022slip}. 
% Finally, there are a number of higher-order effects due to SHSs, discussed in \citep{lee2016superhydrophobic}, such as curvature at the liquid--gas interface and the gas subphase.
% \textit{Explain $A_E^{1D}$ limit.}
% Dashed black asymptotes for $c_0$, $\Gamma_0$ and ${DR}_0$ are plotted when $\alpha\in[10,\,100]$ using \eqref{eq:m_we}--\eqref{eq:d_we} in figure \ref{fig:11}(\textit{a,\,b,\,c,\,d,\,e,\,g}).
% Below, we explore the emergence of 2D effects in regions $M_E^{2D}$ and $A_E^{2D}$, i.e. for $\alpha\ll 1$ and $\delta \ll 1$.
% Correspondingly, the interfacial (bulk) flux increases (decreases) at the upstream end and decreases (increases) at the downstream end of the interface.
% \begin{subequations}
% \begin{align}
% \alpha^{1/3} c_{YY} - \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{1/3}Y\right)\left( \frac{3 \beta}{2 \gamma}+ \frac{\alpha^{2/3}}{\gamma^2} f_x\right)\right)c_x \\ - \frac{\gamma}{\beta}\left(\frac{Y}{2} - \frac{\alpha^{1/3}Y^2}{2}\right)\frac{\alpha^{2/3}}{\gamma^2} f_{xx} c_Y &=0 \quad \text{in} \quad \mathcal{D}_1, \\
% \alpha^{1/3} c_{YY} - \frac{3\alpha^{1/3}Y}{2} c_x &=0  \quad \text{in} \quad \mathcal{D}_2,
% \end{align}
% \end{subequations}
% \begin{subequations} \label{eq:bl_1_m}
% \begin{align}
% C_{YY} - \frac{3Y}{2} C_x + O(\alpha^{1/3}) &=0 \quad \text{in} \quad \mathcal{D}_1, \\
% C_{YY} - \frac{3Y}{2} C_x &=0  \quad \text{in} \quad \mathcal{D}_2.
% \end{align}
% \end{subequations}
% \begin{equation}
%     \alpha^{2/3} c_{Y} - \beta\bigg[\left(\frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \frac{\alpha^{2/3}}{\gamma^2} f_x\right)\right) \left( \frac{3 \beta x}{2 \gamma}+M_1 + \frac{\alpha^{2/3}}{\gamma^2}f\right) \bigg]_x = 0,   
% \end{equation}
% \begin{equation} \label{eq:bl_2_m}
%     C_{Y} - \frac{\gamma}{2}\left[G_x\left(\frac{3\beta x}{2\gamma} + M_1 \right)\right]_x + O(\alpha^{2/3}) = 0.   
% \end{equation}
% \begin{equation}
%     \frac{3}{4}-\frac{\gamma}{2\beta}\Gamma_x =0   
% \end{equation}
% \begin{equation}
%     \frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \frac{\alpha^{2/3}}{\gamma^2}f_x\right) =0   
% \end{equation}
% \begin{subequations}
% \begin{align}
% \beta\left(\frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \frac{\alpha^{2/3}}{\gamma^2}f_x\right)\right) \left(1 + \frac{3 \beta}{2 \gamma}(x+M_1) + \frac{\alpha^{2/3}}{\gamma^2} f_x\right) + \\  \alpha^{1/3}\int_{Y=0}^\infty \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{1/3}Y\right)\left(\frac{3 \beta}{2 \gamma} + \frac{\alpha^{2/3}}{\gamma^2}f_x\right)\right)\left(c-1\right) \, \text{d}Y &= 0, \\
% \int_{x=-\phi}^\phi c_Y \, \text{d} x &= 0, \\
% \int_{Y=0}^\infty \frac{3Y}{2}\left(c-1\right) \, \text{d}Y &= 0,
% \end{align}
% \end{subequations}
% \begin{subequations}
% \begin{align}
% -\frac{1}{2\gamma}\alpha^{2/3}f_x +  \alpha^{2/3}\int_{Y=0}^\infty \frac{3 Y}{2 }\left(c-1\right) \, \text{d}Y + O(\alpha^{2/3}/\gamma^2) &= 0 \quad \text{in} \quad \mathcal{D}_1, \\
% \int_{x=-\phi}^\phi c_Y \, \text{d} x &= 0 \quad \text{in} \quad \mathcal{D}_1, \\
% \int_{Y=0}^\infty \frac{3Y}{2}\left(c-1\right) \, \text{d}Y &= 0  \quad \text{in} \quad \mathcal{D}_2,
% \end{align}
% \end{subequations}
% We can evaluate the following identities
% \refstepcounter{equation}
% \begin{equation}
%     \int_{\eta =0}^\infty \eta F \, \test{d}\eta = \frac{1}{6^{1/3}\Gamma(4/3)}, \quad \int_{\eta =0}^\infty \eta G \, \test{d}\eta = \frac{3^{5/3}/5}{2^{1/3}\Gamma(1/3)}. \tag{\theequation\textit{a,\,b}}
% \end{equation}
% \begin{equation}
%     \frac{f_x}{\gamma} = \int_{Y=0}^\infty 3 Y\left( \left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)F + \frac{3\beta}{2\gamma}(x+\phi)G\right) \, \text{d}Y  = 0
% \end{equation}
% \begin{equation}
%     \frac{f_x}{\gamma} = \int_{Y=0}^\infty \left(3 \eta(x+\phi)^{2/3}\left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)F + \frac{9\beta \eta}{2\gamma}(x+\phi)^{5/3}G \right)\, \text{d}\eta  = 0
% \end{equation}
% \begin{equation}
%     \frac{f_x}{\gamma} = 3 (x+\phi)^{2/3}\left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta+ \frac{9\beta}{2\gamma}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta G \, \text{d}\eta  = 0
% \end{equation}
% \begin{equation}
%     3 (2\phi)^{2/3}\left(M_1 - \frac{3\beta\phi}{2\gamma} - 1 \right)\int_{Y=0}^\infty \eta F \, \text{d}\eta+ \frac{9\beta}{2}(2\phi)^{5/3} \int_{Y=0}^\infty \eta G \, \text{d}\eta= 0
% \end{equation}
% \begin{multline}
%     f = - \frac{9}{5} (x+\phi)^{5/3}\left(\frac{3\beta}{2}(M_1-\phi) - \gamma \right)\int_{\eta=0}^\infty \eta F \, \text{d}\eta \\ -  \frac{27\beta}{16}(x+\phi)^{8/3} \int_{\eta=0}^\infty \eta G \, \text{d}\eta + M_2,
% \end{multline}
% \begin{multline}
%     G= \int\bigg(\frac{3}{2} (x+\phi)^{2/3}\left(- \frac{3\beta\phi M_2}{2\gamma} + \frac{3\beta\phi}{2\gamma}\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta \\ - \frac{9\beta}{4\gamma}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta\bigg)\bigg/\left(\frac{\gamma}{2}\right)\,\text{d}x.
% \end{multline}
% \begin{multline}
%     G= \int\bigg(\frac{3}{\gamma} (x+\phi)^{2/3}\left(- \frac{3\beta\phi M_2}{2\gamma} + \frac{3\beta\phi}{2\gamma}\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta \\ - \frac{9\beta}{2\gamma^2}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta\bigg)\,\text{d}x.
% \end{multline}
% \begin{equation}
%     G= \int\bigg(\frac{9\beta\phi}{2\gamma^2} (x+\phi)^{2/3}\left(1-M_2\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta - \frac{9\beta}{2\gamma^2}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta\bigg)\,\text{d}x.
% \end{equation}
% \begin{multline} 
%     G= \frac{81\beta\phi}{25\gamma^2} (x+\phi)^{5/3}\int_{Y=0}^\infty \eta F \, \text{d}\eta - \frac{27\beta}{16\gamma^2}(x+\phi)^{8/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta  \\ \vspace{-2cm} + M_3 \equiv \frac{J}{\gamma^2} + M_3,
% \end{multline}
% We can extend the range of validity of the interfacial-concentration field in \eqref{eq:bl_m_gamma} to $\gamma = O(1)$ for $\alpha \ll 1$. 
% In this extension of region $M^\textsl{2D}$, we write 
% \refstepcounter{equation} \label{eq:exp_m_2}
% \begin{equation} 
%     \Gamma = 1 + \frac{3 \beta}{2 \gamma}(x + M_1) - \alpha^{2/3} G(x) + ..., \quad c=C(x,\,Y), \tag{\theequation\textit{a,\,b}}
% \end{equation}
% where $y = \alpha^{1/3} Y$ as before.
% % \begin{subequations}
% % \begin{align}
% % \alpha^{1/3} c_{YY} - \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{1/3}Y\right)\left( \frac{3 \beta}{2 \gamma}+ \alpha^{2/3} f_x\right)\right)c_x \\ - \frac{\gamma}{\beta}\left(\frac{Y}{2} - \frac{\alpha^{1/3}Y^2}{2}\right)\alpha^{2/3} f_{xx} c_Y &=0 \quad \text{in} \quad \mathcal{D}_1, \\
% % \alpha^{1/3} c_{YY} - \frac{3\alpha^{1/3}Y}{2} c_x &=0  \quad \text{in} \quad \mathcal{D}_2,
% % \end{align}
% % \end{subequations}
% % \begin{subequations}
% % \begin{align}
% % c_{YY} - \frac{3Y}{2} c_x + O(\alpha^{1/3}\gamma) &=0 \quad \text{in} \quad \mathcal{D}_1, \\
% % c_{YY} - \frac{3Y}{2} c_x &=0  \quad \text{in} \quad \mathcal{D}_2,
% % \end{align}
% % \end{subequations}
% When we substitute \eqref{eq:exp_m_2} into the boundary-layer equations \eqref{eq:bl_1}--\eqref{eq:bl_6}, we recover the same bulk-surfactant equations \eqref{eq:bl_1_m} at leading order.
% For $x\in[-\phi, \, \phi]$ and $Y=0$, we include the higher-order terms neglected for $\gamma \gg 1$ in the interfacial-surfactant equations \eqref{eq:bl_2}, such that
% % \begin{equation}
% %     \alpha^{2/3} c_{Y} - \beta\bigg[\left(\frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \alpha^{2/3} f_x\right)\right) \left(1 + \frac{3 \beta}{2 \gamma}(x + M_1) + \alpha^{2/3}f\right) \bigg]_x = 0,   
% % \end{equation}
% % \begin{equation}
% %     \alpha^{2/3} c_{Y} - \frac{\gamma}{2 }\bigg[\left(- \alpha^{2/3} f_x\right)\left(1 + \frac{3\beta}{2\gamma}(x+M_1)\right) \bigg]_x + O(\alpha^{4/3}) = 0.   
% % \end{equation}
% \begin{equation}
%     C_{Y} - \left[\frac{\gamma}{2} G_{x}\left(1 + \frac{3\beta}{2\gamma}(x+M_1)\right) \right]_x + O(\alpha^{2/3}) = 0.  
% \end{equation}
% % for $x=\pm\phi$ and $y=0$,
% % \begin{equation}
% %     \frac{3}{4}-\frac{\gamma}{2\beta}\Gamma_x =0   
% % \end{equation}
% % \begin{equation}
% %     \frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \alpha^{2/3}f_x\right) =0   
% % \end{equation}
% % \begin{equation}
% %     f_x =0   
% % \end{equation}
% % for $x\in[\phi, \, 2 - \phi]$ and $y=0$,
% % \begin{equation} 
% % 	c_{Y} =0,
% % \end{equation}
% % and for $x\in[-\phi, \, 2 - \phi]$ and $y\rightarrow\infty$,
% % \begin{equation} 
% % 	c = 1.
% % \end{equation}
% The no-flux and core conditions remain as in \eqref{eq:bl_3_m}--\eqref{eq:bl_5_m}.
% The excess-surfactant-flux conditions \eqref{eq:bl_6} also include higher-order terms neglected for $\gamma \gg 1$ and are given by
% % \begin{subequations}
% % \begin{align}
% % \beta\left(\frac{3}{4}-\frac{\gamma}{2\beta}\left(\frac{3 \beta}{2 \gamma} + \alpha^{2/3}f_x\right)\right) \left(1 + \frac{3 \beta}{2 \gamma}(x+M_1) + \alpha^{2/3} f_x\right) + \\  \alpha^{1/3}\int_{Y=0}^\infty \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{1/3}Y\right)\left(\frac{3 \beta}{2 \gamma} + \alpha^{2/3}f_x\right)\right)\left(c-1\right) \, \text{d}Y &= 0, \\
% % \int_{x=-\phi}^\phi c_Y \, \text{d} x &= 0, \\
% % \int_{Y=0}^\infty \frac{3Y}{2}\left(c-1\right) \, \text{d}Y &= 0,
% % \end{align}
% % \end{subequations}
% % \begin{subequations}
% % \begin{align}
% % -\frac{\gamma}{2}\alpha^{2/3}f_x\left(1 + \frac{3\beta}{2\gamma}(x + M_1)\right) +  \alpha^{2/3}\int_{Y=0}^\infty \frac{3 Y}{2 }\left(c-1\right) \, \text{d}Y + O(\alpha^{4/3}) &= 0, \\
% % \int_{x=-\phi}^\phi c_Y \, \text{d} x &= 0 , \\
% % \int_{Y=0}^\infty \frac{3Y}{2}\left(c-1\right) \, \text{d}Y &= 0 ,
% % \end{align}
% % \end{subequations}
% \begin{subequations} \label{eq:bl_6_m_2}
% \begin{align}
% \int_{Y=0}^\infty \frac{3 Y}{2 }\left(C-1\right) \, \text{d}Y + \frac{\gamma}{2} G_x\left(1 + \frac{3\beta}{2\gamma}(x+M_1)\right) + O(\alpha^{2/3}) &= 0 \quad \text{in} \quad \mathcal{D}_1, \\
% \int_{x=-\phi}^\phi C_Y \, \text{d} x &= 0 \quad \text{in} \quad \mathcal{D}_1, \\
% \int_{Y=0}^\infty \frac{3Y}{2}\left(C-1\right) \, \text{d}Y &= 0  \quad \text{in} \quad \mathcal{D}_2.
% \end{align}
% \end{subequations}

% The construction of the similarity solution for $C$ in region $M^\textsl{2D}$ remains as is defined in \eqref{eq:ss_m}, with $F$ and $H$ given in \eqref{eq:FandG}, and the similarity variable $\eta = Y/(x+\phi)^{1/3}$.
% % \begin{equation}
% %     c = 1 + \left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)F(\eta) + \frac{3\beta}{2\gamma}(x+\phi)G(\eta)
% % \end{equation}
% % with $\eta = Y/(x+\phi)^{1/3}$ and 
% % \begin{equation}
% %     F'' + \frac{\eta^2}{2}F = 0, \quad F(0)=1, \quad F(\infty) =0,   
% % \end{equation}
% % \begin{equation}
% %     G'' + \frac{\eta^2}{2}G - \frac{3}{2}G = 0, \quad G(0)=1, \quad G(\infty) =0.   
% % \end{equation}
% % These have the solution
% % \refstepcounter{equation}
% % \begin{equation}
% %     F = \frac{\Gamma(1/3, \, \eta^3/6)}{\Gamma(1/3)}, \quad G = \frac{ (4 + \eta^3) \mathrm{\Gamma}(1/3, \, \eta^3/6) -6^{2/3} \eta \exp(-\eta^3/6) }{4 \Gamma(1/3)}, \tag{\theequation\textit{a,\,b}}
% % \end{equation}
% % where we can evaluate
% % \refstepcounter{equation}
% % \begin{equation}
% %     \int_{\eta =0}^\infty \eta F \, \test{d}\eta = \frac{1}{6^{1/3}\Gamma(4/3)}, \quad \int_{\eta =0}^\infty \eta G \, \test{d}\eta = \frac{3^{5/3}/5}{2^{1/3}\Gamma(1/3)}. \tag{\theequation\textit{a,\,b}}
% % \end{equation}
% Substituting the bulk concentration \eqref{eq:ss_m} into the surfactant-flux conditions \eqref{eq:bl_6_m_2}, we have
% % \begin{multline}
% %     \gamma f_x\left(1+\frac{3\beta}{2\gamma}(x+M_1)\right) \\ = \int_{Y=0}^\infty 3 Y\left( \left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)F + \frac{3\beta}{2\gamma}(x+\phi)G\right) \, \text{d}Y  = 0
% % \end{multline}
% % \begin{multline}
% %     \gamma f_x\left(1+\frac{3\beta}{2\gamma}(x+M_1)\right) \\ = \int_{Y=0}^\infty \left(3 \eta(x+\phi)^{2/3}\left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)F + \frac{9\beta \eta}{2\gamma}(x+\phi)^{5/3}G \right)\, \text{d}\eta  = 0
% % \end{multline}
% % \begin{multline}
% %     \gamma f_x\left(1+\frac{3\beta}{2\gamma}(x+M_1)\right) \\ = 3 (x+\phi)^{2/3}\left(\frac{3\beta}{2\gamma}(M_1-\phi)-1\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta+ \frac{9\beta}{2\gamma}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta G \, \text{d}\eta  = 0
% % \end{multline}
% \begin{multline} \label{eq:bl_g_x}
%     \gamma G_x\left(1+\frac{3\beta}{2\gamma}(x+M_1)\right) = - 3 (x+\phi)^{2/3}\left(\frac{3\beta}{2}(M_1-\phi) - \gamma \right)\int_{Y=0}^\infty \eta F \, \text{d}\eta \\ - \frac{9\beta}{2}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta.
% \end{multline}
% When we integrate \eqref{eq:bl_g_x} in $x$ and employ the no-flux condition \eqref{eq:bl_3_m} at $x=\phi$, we recover the same $M_1$ and $\widetilde{M}_1$ defined in \eqref{eq:bl_m_def} and derived for $\gamma \gg 1$.
% % \begin{equation}
% %     3 (2\phi)^{2/3}\left(\frac{3\beta}{2}(M_1-\phi) - \gamma \right)\int_{Y=0}^\infty \eta F \, \text{d}\eta+ \frac{9\beta}{2}(2\phi)^{5/3} \int_{Y=0}^\infty \eta G \, \text{d}\eta= 0
% % \end{equation}
% % \begin{equation}
% %     M_1 = \frac{\phi\left(\left(1 - \frac{2\gamma}{3\beta\phi}\right)\int_{Y=0}^\infty \eta F \, \text{d}\eta- 2 \int_{Y=0}^\infty \eta G \, \text{d}\eta\right)}{\int_{Y=0}^\infty \eta F \, \text{d}\eta}.
% % \end{equation}
% % \begin{equation}
% %     M_1 = \frac{\phi\left(\int_{Y=0}^\infty \eta F \, \text{d}\eta- 2 \int_{Y=0}^\infty \eta G \, \text{d}\eta\right)}{\int_{Y=0}^\infty \eta F \, \text{d}\eta} + \frac{2\gamma}{3\beta}.
% % \end{equation}
% We can then integrate \eqref{eq:bl_g_x} again in $x$ to give the correction to the immobilised solution for the interfacial concentration
% \begin{multline}
%     G = - \int \bigg\{ \bigg(\frac{9\beta}{2} (x+\phi)^{2/3}(\widetilde{M}_1-\phi)\int_{Y=0}^\infty \eta F \, \text{d}\eta + \frac{9\beta}{2}(x+\phi)^{5/3} \int_{Y=0}^\infty \eta H \, \text{d}\eta \bigg) \\ \bigg/ \left(\gamma+\frac{3\beta}{2}(x+M_1)\right)\bigg\}\,\text{d}x,
% \end{multline}
% Hence, in this extension of $M^\textsl{2D}$ to $\gamma = O(1)$,
% the interfacial concentration becomes
% \begin{equation} \label{eq:gam_ext}
%     \Gamma = 1 + \frac{3\beta}{2\gamma}(x + M_1) -\alpha^{2/3} G(x; \beta, \, \gamma, \, \phi).
% \end{equation}
% Then substituting \eqref{eq:gam_ext} into \eqref{eq:dr_def}, the leading-order drag reduction is given by 
% \begin{equation}
%     {DR}_0 = \frac{\gamma \alpha^{2/3} \Delta G(\beta,\,\gamma,\,\phi)}{3\phi\beta} \equiv m_2 \alpha^{2/3}.
% \end{equation}
% [Explain how interfacial diffusion allows $u_0$ to be non-zero at $x=-\phi$.]  
% Above the quasi-stagnant region, streamlines are tilted, particularly at its leading edge.
% The upward vertical flow pushes some surfactant away from the interface towards the core of the channel. 
% A scaling argument defining the asymptotic regions is as follows ($\sim$ denotes `scales like'). 
% \begin{itemize}
% \item In the slip region ($-\phi<x<x_0$),  $x\sim 1$, $y\sim \alpha^{1/2}$; $C$ varies by $O(1)$ across the boundary layer so that $C_y\sim \alpha^{-1/2}$.  This delivers a flux per unit length $\alpha C_y\sim \alpha^{1/2}$ to the interface, allowing $\Gamma$ to grow to $O(\alpha^{1/2})$.  The bulk concentration field is zero at the interface to leading order, and is coupled to $\Gamma$ through an $O(\alpha^{1/2})$ correction.  This region delivers an interfacial flux of $O(\alpha^{1/2})$ at its outlet.
% \item In the deceleration region ($x$ very close to $x_0$), $u$ varies by $O(1)$ over a short horizontal scale and $\Gamma\sim\alpha^{1/2}$.  Thus $x\sim \gamma\alpha^{1/2}$ for $u_s$ to balance $\gamma \Gamma_x$.  Diffusion balances advection by $u$ over a vertical lengthscale $y\sim (\alpha x)^{1/2}\sim \gamma^{1/2}\alpha^{3/4}$.  Diffusion influences the concentration field where the field is $O(\alpha^{1/2})$ in magnitude, near the interface; advection dominates transport in the upper part of the boundary layer.  At the downstream limit of this region, $u$ falls towards zero, with $\Gamma_x\approx 3\beta/(2\gamma)$.  The region is too short for there to be appreciable desorption, so flux conservation requires that $u\sim \alpha^{1/2}/\Gamma\sim\alpha^{1/2} \gamma/(x-x_0)\ll 1$ at the region's outlet.
% \item In the transition region ($x$ close to $x_0$), there is a balance in the bulk between vertical diffusion, advection by $u$ (which is now $o(1)$) and advection by shear, {\hbox{i.e.}} $\alpha/y^2\sim u/x\sim y/x$; thus $y\sim u\sim (\alpha x)^{1/3}$.  Matching $u$ to the deceleration region requires $u\sim \alpha^{1/2}\gamma/x$, implying $x\sim \gamma^{3/4}\alpha^{1/8}$, $y\sim u\sim\gamma^{1/4}\alpha^{3/8}$.  $\Gamma$ is linear at leading order ($\Gamma\approx 3\beta(x-x_0)/(2\gamma)$ with a correction $\sim u x/\gamma\sim \alpha^{1/2}$; the bulk concentration is set by the dominant interfacial concentration, and is $O(x/\gamma)\sim \alpha^{1/8}/\gamma^{1/4}$.  The region is again too short for there to be appreciable desorption, so the interfacial flux is still $O(\alpha^{1/2})$.  Advection dominates transport in the boundary layer for large $y$.
% \item The quasi-stagnant region ($x_0<x<\phi$) has a length $L=\phi-x_0$ that is yet to be determined.  $\Gamma$ is again linear (with slope $1/\gamma$) with a correction to be determined.   This sets the bulk and interfacial concentration scales as $L/\gamma$.  In the bulk, diffusion balances shear over a vertical lengthscale $y\sim (\alpha L)^{1/3}$.  Thus $\alpha C_y\sim \alpha (L/\gamma) (\alpha L)^{-1/3}\sim (\alpha L)^{2/3}/\gamma$.  Integrated over a lengthscale $L$,  this accommodates the $O(\alpha^{1/2})$ interfacial flux, so that $L\sim \gamma^{3/5}/\alpha^{1/10}$.   The drag generated by the monolayer is proportional to $\gamma \Delta \Gamma\sim L$.
% \end{itemize}
% This analysis does not extend up to the limit $\gamma=O(1)$ where region $M^{2D}$ begins.
% is not strongly met for $\alpha=0.1$, $\gamma=0.1$.  Formally, we expect DR contours in the $(\log \alpha,\log \gamma)$ plane to have slope 1/6 in the limit when these lengthscales become distinct.  
% \subsubsection{$\mathcal{D}_2$}

% A dipolar field with $C>C_\mathrm{I}$ ($C<C_{\mathrm{I}}$) in the lower (upper) part of the boundary layer enters $\mathcal{D}_2$.   Defining $A=\int_0^\infty (C-C_{\mathrm{I}})y^4\,\mathrm{d}y$, and noting (\ref{eq:d2}), 
% \begin{multline}
% A_x=\int_0^\infty C_x y^4\,\mathrm{d}y=\frac{2\alpha}{3} \int_{0}^\infty y^3 C_{yy} \,\mathrm{d}y=\frac{2\alpha}{3} \left([y^3 C_y ]_0^\infty-3\int_0^\infty y^2 C_y\,\mathrm{d}y\right) \\
% =-{2\alpha} \left([y^2 (C-C_{\mathrm{I}} ]_0^\infty-2 \int_0^\infty y (C-C_{\mathrm{I}})\,\mathrm{d}y\right).
% \end{multline}
% Thus provided $\int_0^\infty y(C-C_{\mathrm{I}})\,\mathrm{d}y=0$, $A$ is uniform along $\mathcal{D}_2$ under the shear flow.   A localised source at the inlet to $\mathcal{D}_2$ would have a boundary layer growing in thickness like $(\alpha x)^{1/3}$ and we would expect the concentration to decay proportionally to $x^{-5/3}$.  We assume that this decay is sufficiently quick for $C\approx C_\mathrm{I}$ at the inlet to region $\mathcal{D}_1$.
% \begin{subequations} 
% \begin{align}
% c_{YY} - \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{1/2}Y\right)\alpha^{1/2}G_x\right)c_x - \frac{\gamma}{\beta}\left(\frac{\alpha^{1/2}Y}{2} - \frac{\alpha Y^2}{2}\right)G_{xx} c_Y &=0.
% \end{align}
% \end{subequations}
% \begin{equation} \label{eq:bl_1_a}
% C_{YY} - \frac{3}{4} C_x + O(\alpha^{1/2}\gamma) =0.
% \end{equation}
% \begin{equation}
%     \alpha^{1/2} c_{Y} = \beta\bigg[\left(\frac{3}{4}-\frac{\gamma}{2\beta}\alpha^{1/2}G_x\right) \alpha^{1/2}G \bigg]_x.   
% \end{equation}
% \begin{equation} \label{eq:bl_2_a} 
%     C_{Y} = \frac{3\beta}{4} G_x + O(\alpha^{1/2}\gamma).  
% \end{equation}
% We assume that the length of the slip region is much larger than the boundary-layer thickness and there is no interaction between the asymptotic regions labelled in figure \ref{fig:asym_shems}(\textit{b}). 
% \begin{multline} 
% \frac{\alpha^{3/2} \lambda}{\gamma \alpha^{3/2}} C_{YY} - \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \gamma^{1/2}\alpha^{3/4}Y\right)\frac{\alpha^{1/2}\lambda}{\gamma\alpha^{1/2}}G_X\right)\frac{\alpha^{1/2}\lambda}{\gamma\alpha^{1/2}} C_X \\ - \frac{\gamma}{\beta}\left(\frac{\gamma^{1/2}\alpha^{3/4}Y}{2} - \frac{\gamma\alpha^{3/2} Y^2}{2}\right)\frac{\alpha^{1/2}\lambda}{\gamma^2 \alpha}G_{XX} \frac{\alpha^{1/2}\lambda}{\gamma^{1/2}\alpha^{3/4}}C_Y =0.
% \end{multline}
% \begin{multline} 
% C_{YY} - \left(\frac{3}{4}+\frac{1}{\beta}\left(-\frac{1}{2} + \gamma^{1/2}\alpha^{3/4}Y\right)\lambda G_X\right) C_X \\ - \frac{1}{\beta}\left(\frac{Y}{2} - \frac{\gamma^{1/2}\alpha^{3/4} Y^2}{2}\right)G_{XX}\lambda C_Y =0.
% \end{multline}
% \begin{equation}  \label{eq:bl_1_a_dec}
% C_{YY} - \left(\frac{3}{4}-\frac{\lambda}{2\beta} G_X\right) C_X  - \frac{\lambda Y}{2 \beta}G_{XX} C_Y + O(\gamma^{1/2}\alpha^{3/4})=0.
% \end{equation} 
% \begin{equation}
%     \alpha^{1/2} c_{Y} = \beta\bigg[\left(\frac{3}{4}-\frac{\gamma}{2\beta}\alpha^{1/2}G_x\right) \alpha^{1/2}G \bigg]_x.   
% \end{equation}
% \begin{equation} \label{eq:bl_2_a_dec} 
%     \left[\frac{3}{4}G - \frac{\lambda}{2\beta} G_X G\right]_X + O(\gamma^{1/2}\alpha^{3/4})  = 0.
% \end{equation}
% Above this small region, in which advection and diffusion balance, we expect advection to dominate diffusion. 
% Over the same streamwise lengthscale, we can consider the large-$Y$ limit of (\ref{eq:qs1}).  
% Here, $UF_X- U_XY F_Y=0$ is satisfied by $F=F_0(\psi)$ where $\psi=YU(X)$ (\hbox{i.e.}, the concentration is constant along streamlines).  
% \begin{multline}
%     \alpha \frac{\alpha^{1/8}}{\gamma^{1/4}} \frac{1}{\alpha^{6/8} \gamma^{2/4}} C_{YY} \\ - \left(\frac{3}{4}+\frac{\gamma}{\beta}\left(-\frac{1}{2} + \alpha^{3/8}\gamma^{1/4}Y\right)\left(\frac{3\beta}{2\gamma} + \alpha^{1/2}\frac{1}{\alpha^{1/8}\gamma^{3/4}} G_X\right)\right)\frac{\alpha^{1/8}}{\gamma^{1/4}} \frac{1}{\alpha^{1/8}\gamma^{3/4}} C_X \\
%     - \frac{\gamma}{\beta}\left(\frac{y}{2} - \frac{y^2}{2}\right)\Gamma_{xx} c_y =0
% \end{multline}
% \begin{multline}
%     \frac{\alpha^{3/8}}{\gamma^{3/4}} C_{YY} - \left(\frac{3}{4}+\frac{1}{\beta}\left(-\frac{1}{2} + \alpha^{3/8}\gamma^{1/4}Y\right)\left(\frac{3\beta}{2\gamma} + \frac{\alpha^{3/8}}{\gamma^{3/4}} G_X\right)\right) C_X \\
%     - \frac{\gamma}{\beta}\left(\frac{y}{2} - \frac{y^2}{2}\right)\Gamma_{xx} c_y =0
% \end{multline}
% \begin{equation} 
% \label{eq:transbulk}
% C_{YY} + \left(\frac{G_X}{2\beta} -\frac{3Y}{2} \right)C_X- \frac{G_{XX}}{2\beta} Y C_Y + O(\alpha^{3/8}\gamma^{1/4}) = 0.
% \end{equation}
% \refstepcounter{equation} \label{eq:transout}
% \begin{multline}
% \Gamma\approx \frac{3\beta(x-x_0)}{2\gamma} +\alpha^{1/2}\left[ -\lambda \log\left(\frac{x-x_0}{\alpha^{1/8} \gamma^{3/4}}\right) +B\right]+..., \\ u(x,\,0)=\frac{\lambda \alpha^{1/2}\gamma}{2\beta(x-x_0)}+..., \tag{\theequation\textit{a,\,b}}
% \end{multline}
% Again, for large $Y$ values, we expect diffusion to be subdominant to advection in (\ref{eq:transbulk}) and for concentration to be constant along streamlines with constant $\psi=\lambda Y/(2\beta X)+\tfrac{3}{4}Y^2$; the shear bends streamlines in the flow direction.
% \begin{equation}
% \beta \left[ u_s \frac{3\beta}{2\gamma}(x-x_0) \right]_x+O(1) = \frac{\alpha}{(\alpha(x-x_0)^{1/3}} \frac{3\beta}{2\gamma}(x-x_0) C'(0).
% \end{equation}
% \begin{equation} \label{eq:bl_2_qs}
% \beta \left[ u(x,\,0)(x-x_0) \right]_x+O(\gamma) = (\alpha(x-x_0))^{2/3}C'(0).
% \end{equation}
% \begin{equation}
% \beta  u_s = \frac{3\alpha^{2/3} C'(0)}{5}(x-x_0)^{5/3} + A_2
% \end{equation}
% \begin{equation}
% 0 = \frac{3\alpha^{2/3} C'(0)}{5}(\phi-x_0)^{5/3} + A_2
% \end{equation}
% \begin{equation}
% u_s = - \frac{3\alpha^{2/3} C'(0)}{5\beta } \left(\frac{(\phi-x_0)^{5/3}}{x-x_0}-(x-x_0)^{2/3}\right) = \frac{\lambda \alpha^{1/2}\gamma}{2\beta(x-x_0)}.
% \end{equation}
% \begin{equation}
% \Gamma_{\max}\approx \frac{3\beta}{2} \left[ \frac{5\lambda}{6 [-F_\eta(0)]} \right]^{3/5}\frac{1}{(\alpha\gamma^4)^{1/10}}.
% \end{equation}
% Check that (\ref{eq:findx0}) ensures that net adsorption balances net desorption in (\ref{eq:netades}); (\ref{eq:findx0}) specifies $x_0$.   
% The correction to the surfactant field is obtained by integrating $\gamma G_x/(2\beta)=-u_s$, giving
% \begin{equation}
% G\approx \frac{6\alpha^{1/3}}{5\gamma} [-F_\eta(0)](\phi-x_0)^{5/3}\log (x-x_0)  
% \end{equation}
% Check the match to (\ref{eq:transout}) and subdominance to $3\beta(x-x_0)/2\gamma$.
% The flux $\beta u_s \Gamma$ is predicted to be proportional to $(\phi-x_0)^{5/3}-(x-x_0)^{5/3}$ in the QS region.
% \begin{equation}
%     {DR}_0 = 1 - \frac{\gamma}{3\beta\phi}\frac{3\beta}{2} \left[ \frac{5\lambda}{6 [-F_\eta(0)]} \right]^{3/5}\frac{1}{(\alpha\gamma^4)^{1/10}}
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \int_{x_0}^\phi \left[u_s \frac{3\beta}{2\gamma}(x-x_0)\right]_x \,\text{d}x
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \int_{x_0}^\phi \left[- \frac{9 \alpha^{2/3} \beta C'(0)}{10\gamma} \left( (\phi-x_0)^{5/3} -(x-x_0)^{5/3}\right)\right]_x \,\text{d}x
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \left[- \frac{9 \alpha^{2/3} \beta C'(0)}{10\gamma} \left( (\phi-x_0)^{5/3} -(x-x_0)^{5/3}\right)\right]_{x=x_0}^\phi 
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = - \frac{9 \alpha^{2/3} \beta C'(0)}{10\gamma} \left( (\phi-x_0)^{5/3} -(\phi-x_0)^{5/3} - (\phi-x_0)^{5/3} \right) 
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \frac{9 \alpha^{2/3} \beta C'(0)}{10\gamma} (\phi-x_0)^{5/3} 
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \frac{9 \alpha^{2/3} \beta C'(0)}{10\gamma} \left(\frac{5 \lambda \gamma}{-6\alpha^{1/6}C'(0)} \right)
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \frac{9 \alpha^{2/3} \beta C'(0)}{10} \left(\frac{5}{-6\alpha^{1/6}C'(0)} \right) \frac{4}{\beta}\left(\frac{x_0+\phi}{3\pi}\right)^{1/2}
% \end{equation}
% \begin{equation}
%     \int_{x_0}^\phi c_y(x,\,0)\,\text{d}x = \frac{9}{10} \left(\frac{5}{-6} \right) 4 \left(\frac{\alpha^{1/2}(x_0+\phi)}{3\pi}\right)^{1/2}
% \end{equation}
% At $O(1)$, advection and Marangoni effects dominate in the bulk surfactant equations \eqref{eq:bl_1}, such that
% \begin{subequations} 
% \label{eq:ame_1}
% \begin{align}
% 	- \left(\frac{3}{4} + \frac{\gamma}{\beta} \left(-\frac{1}{2} + y \right) G_{0x}\right) C_{0x} - \frac{\gamma}{\beta} \left(\frac{y}{2} - \frac{y^2}{2}\right) G_{0xx} C_{0y} &= 0 \quad \text{in} \quad \mathcal{D}_1, \\
%     - \left(\frac{3y}{2} \right) C_{0x} &= 0 \quad \text{in} \quad \mathcal{D}_2.
% \end{align}
% \end{subequations} 
% The no-flux of bulk surfactant condition \eqref{eq:c_bvp_4_wd} gives, for $x\in[\phi, \, 2 - \phi]$ and $y=0$ (and for $x\in[-\phi, \, 2-\phi]$ and $y=2$)  
% \begin{equation} \label{eq:ame_4} 
% 	c_{00y} =0.
% \end{equation}
% There is no forcing in the bulk-concentration problem (\ref{eq:ame_1}, \ref{eq:ame_2}\textit{a}, \ref{eq:ame_4}, \ref{eq:ame_5}, \ref{eq:ame_6}), so we assume that the bulk concentration is constant in the channel to leading order.
% Using the surfactant-flux conditions \eqref{eq:ame_5}--\eqref{eq:ame_6}, we then have that $c_{00} = 1$ (the interfacial flux is zero using (\ref{eq:ame_2}\textit{a})--\eqref{eq:ame_4}, the first term in the bulk flux integrates to $c_{00}$ and the second term in the bulk flux integrates to zero).
% The expression for leading-order drag reduction \eqref{eq:dr_am} was derived using asymptotic approximations for weak cross-channel diffusion and bulk--surface exchange.
% Hence, ${DR}_0 = \text{constant}$ for $\gamma = O(\beta)$ when bulk--surface exchange is weak, such that the drag increases with increasing $\gamma$.

